Beating the random assignment on constraint satisfaction problems of bounded degree

We show that for any odd $k$ and any instance of the Max-kXOR constraint satisfaction problem, there is an efficient algorithm that finds an assignment satisfying at least a $\frac{1}{2} + \Omega(1/\sqrt{D})$ fraction of constraints, where $D$ is a bound on the number of constraints that each variable occurs in. This improves both qualitatively and quantitatively on the recent work of Farhi, Goldstone, and Gutmann (2014), which gave a \emph{quantum} algorithm to find an assignment satisfying a $\frac{1}{2} + \Omega(D^{-3/4})$ fraction of the equations. For arbitrary constraint satisfaction problems, we give a similar result for "triangle-free" instances; i.e., an efficient algorithm that finds an assignment satisfying at least a $\mu + \Omega(1/\sqrt{D})$ fraction of constraints, where $\mu$ is the fraction that would be satisfied by a uniformly random assignment.

==> content/3lin.tex <==
%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

\section{Bounded degree \maxthreelin}

A \maxthreelin instance $\inst$ is a constraint system $\{P_\ell\}_{\\ell \in
  [m]}$ where each predicate $P_\ell$ is on exactly $3$ variables and
is of the form $P_\ell(x_{S_\ell}) = \frac{1}{2} (1 + b_\ell \prod_{i \in S_\ell}
x_i)$ for some $b_\ell \in \sbits$.

Equivalently, the instance $\inst$ of \maxthreelin corresponds to a
degree $3$ polynomial as described below.
$$ \inst(x) = \frac{1}{2} + \frac{1}{2m} \cdot \sum_{i,j,\ell \in [n]} a_{ij\ell} x_ix_jx_\ell \mcom$$
where $a_{ijk} = a_{ikj} = a_{jik} = a_{jki} = a_{kij} = a_{kji} = \frac{b_{\ell}}{6}$ if there is a constraint $x_i x_j x_k =
b_\ell$ and $0$ otherwise.  We will also set $a_{iij} = a_{iji} = a_{jii}
= 0$ for all $i,j \in [n]$.


\begin{theorem}
  There is an efficient algorithm that given an instance $\inst$ of \maxthreelin where the degree of each
  variable is at most $d$, outputs an assignment $x \in \sbits^n$ such that,
$$ \E\inst(y)  \geq \frac{1}{2} +  \frac{1}{180 d^{1/2}} $$
\end{theorem}
\begin{proof}
First, we will construct from the instance $\inst$, a tripartite
instance $\inst'$ of \maxthreelin.  The tripartite instance $\inst'$
has three sets of variables $\{x_i\}_{i\in [n]}, \{y_j\}_{j\in [n]}$
and $\{z_k\}_{k\in [n]}$.  Moreover, for every constraint $x_ix_jx_k = b_{ijk}$
in the instance $\inst$ we will include $6$ constraints in $\inst'$ of
the following form:
$$x_iy_jz_k = x_i y_kz_j = x_jy_iz_k = x_j y_kz_i = x_ky_iz_j = x_k y_jz_i = b_{ijk}$$

The above described reduction to tripartite instance of \maxthreelin is due to the
work of Khot and Naor \cite{KN08}.  We reproduce Lemma 2.1 from
\cite{KN08} below.

\begin{lemma}  For all $\{a_{ijk}\}_{i,j,k\in[n]}$ such that $a_{iij} =
  a_{jii} = a_{iji} = 0$ for all $i,j \in [n]$,
  $$ \frac{1}{10}\max_{x,y,z \in \sbits^n} \sum_{i,j,k \in [n]} a_{ijk} x_i y_j
  z_k \leq \max_{x \in \sbits^n} \sum_{i,j,k \in [n]} a_{ijk}x_ix_jx_k
  \leq \max_{x \in \sbits^n} \sum_{i,j,k \in [n]} a_{ijk}x_iy_jz_k$$

Furthermore, there exists an efficient randomized procedure that takes
an assignment $x,y,z \in \sbits^n$ to yields an assignment $x \in
\sbits^n$ whose value is bounded as above.
\end{lemma}

Given the tripartite instance $\inst'$, we will construct an
assignment $x,y,z \in \sbits^n$ using the following randomized procedure.
%
\begin{mybox}
  \begin{itemize}
    \item Sample $x,y \in \sbits^n$ uniformly at random.
      \item For each $\ell \in [n]$, set
       $$ z_{\ell} \defeq \sign\left(\sum_{i,j \in [n]} a_{ij\ell}x_iy_j\right)$$
    \end{itemize}
\end{mybox}
%
Now we are ready to lower bound the expected value
of the assignment $x,y,z$ on instance $\inst'$.

\begin{align*}
\E\inst'(x,y,z) &= \frac{1}{2} + \frac{1}{2m} \cdot \E\sum_{i,j,\ell \in [n]}
  a_{ij\ell}x_iy_j z_\ell \\
&= \frac{1}{2} + \frac{1}{2m }\sum_{\ell \in  [n]} \E\left|\sum_{ij} a_{ij\ell} x_i y_j\right| \\
&\geq \frac{1}{2} + \frac{1}{2m} \cdot \sum_{\ell \in  [n]}  \frac{1}{9} \left( \E (\sum_{ij\ell} a_{ij\ell} x_i y_j)^2
  \right)^{1/2} \text{ using \pref{fact:khinchine-poly} for degree 2 polynomials}\\
& = \frac{1}{2}+ \frac{1}{18m} \sum_{\ell \in [n]} \left(\sum_{\ell \in [n]} a^2_{ij\ell}\right)^{1/2}\\
& = \frac{1}{2}+ \frac{1}{18m} \sum_{\ell \in [n]} \left(\card{N(\ell)}\right)^{1/2}\\
& = \frac{1}{2}+ \frac{1}{18} \cdot \frac{\sum_{\ell \in [n]} \left(\card{N(\ell)}\right)^{1/2}}{\sum_{\ell \in [n]}
  \card{N(\ell)}} \qquad (\text{ using } \sum_{\ell \in
  [n]}\card{N(\ell)} > m)\\
& = \frac{1}{2} + \frac{1}{18 \sqrt{d}}  \qquad (\text{using } \card{N(\ell)} \leq d)
\end{align*}
%First, we show the following lower bound on the value of an assignment
%output by the algorithm.
%\begin{claim} \label{lem:degreethreepoly}
%  For every degree $3$ polynomial $A(x,y,z) = \sum_{ij\ell} a_{ij\ell}
%  x_i y_j z_\ell$, the assignment output by the above algorithm satisfies,
%$$ \E\sum_{i,j,\ell \in [n]} a_{ij\ell} x_i y_j z_\ell \geq \sum_{\ell \in
%[n]} \left( \sum_{ij} a_{ij\ell}^2 \right)^{1/2}$$
%\end{claim}
%
%\begin{proof}
%By definition of the assignment $x,y,z$,  we have
%\begin{align*}
%\E\sum_{i,j,\ell \in [n]} a_{ij\ell}x_iy_j z_{\ell}
%&= \sum_{\ell \in  [n]} \E\left|\sum_{ij} a_{ij} x_i y_j\right| \\
%&\geq \sum_{\ell \in  [n]}  \frac{1}{9} \left( \E (\sum_{ij\ell} a_{ij\ell} x_i y_j)^2
%  \right)^{1/2} \text{ using \pref{fact:khinchine-poly} for degree 2 polynomials}\\
%& = \frac{1}{9} \sum_{\ell \in [n]} \left(\sum_{\ell \in [n]} a^2_{ij\ell}\right)^{1/2}
%\end{align*}
%\end{proof}
%

\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% OLD STUFF
\iffalse
\begin{mybox}
  \begin{itemize}
    \item Sample $x \in \sbits^n$ uniformly at random.
      \item For each $i \in [n]$ and $\ell \in N(i)$, set
        $$ s_i(\ell) \defeq \Delta_i P_\ell (x) = b_\ell \cdot \prod_{j \in S_{\ell} \backslash \{i\}} x_j\mcom$$
and let
$$s_i \defeq \sign\left( \sum_{\ell \in N(i)}s_{i}(\ell)\right) \mper$$

\item Output an assignment $y \in \sbits^n$ sampled by fixing for each $i
  \in [n]$ independently,
  $$ y_i \defeq \begin{cases} x_i & \text{ with probability } 1-\e\\
  s_i & \text{ with probability} \e
  \end{cases}$$
  where $\e = \frac{1}{6 d^{1/4} }$
    \end{itemize}
\end{mybox}

\begin{proof}
\begin{align}
 \E_{\ell \in [m]} \E\left[ P_\ell(y_{S_\ell}) \right] & = \E_{\ell \in [m]}
                                                   \sum_{A \cup B \sse S_\ell}
                                                   \e^{\card{A}}(1-\e)^{\card{B}}
                                                   P_\ell(s_A,
                                                   x_B)  \nonumber \\
  &= \frac{1}{2} +  \E_{\ell \in [m]}
                                                   \sum_{\substack{
A \cup B \sse S_\ell, \\
    }}
                                                   \e^{\card{A}}(1-\e)^{\card{B}}
                                                   \left(P_\ell(s_A,
                                                   x_B) -
    \frac{1}{2} \right) \label{eq:lin123}
\end{align}
Here the sum is over all possible partitions of $S_\ell$ in to $A \cup B$.
We will bound terms for each value of $\card{A}$ separately.  First, observe that the terms where $A = \emptyset$ correspond to,
\begin{align*}
   \E_{\ell \in [m]}
                                                   \sum_{\substack{
A \cup B \sse S_\ell, \\
    A = \emptyset}}
                                                   \e^{\card{A}}(1-\e)^{\card{B}}
                                                   \left(P_\ell(s_A,
                                                   x_B) -
    \frac{1}{2} \right) =   \E_{\ell \in [m]} (1-\e)^{3} \left(P_\ell(x_{S_\ell}) - \frac{1}{2} \right)  = 0 \label{eq:nosignal} \mcom
\end{align*}
where we used the fact that $\E P_\ell(x_{S_\ell}) = \frac{1}{2}$.

The crucial positive contribution to the number of satisfied clauses
is from terms with $|A| = 1$.  Specifically, we can write,
\begin{align}
 \E_{\ell \in [m]} \sum_{\substack{A \cup B \sse S_\ell, \\ \card{A} = 1}} \left(P_\ell(s_A, x_B) - \frac{1}{2} \right)
%
&= \frac{1}{m}  \sum_{i \in [n]} \sum_{\ell \in N(i)} \E \left[  P_\ell(s_i,x_{S_\ell
                        \backslash\{i\}})- \frac{1}{2} \right]\nonumber\\
%
&= \frac{1}{2m}  \sum_{i \in [n]} \sum_{\ell \in N(i)}  \E \left[ s_i \cdot \left( b_i\prod_{j \in
  S_{\ell}\backslash \{i\}}x_{j}\right)\right]  \nonumber\\
&= \frac{1}{2m}  \sum_{i \in [n]} \E \left[ s_i \cdot \left(  \sum_{\ell \in N(i)}   \Delta_i P_\ell\right) \right] \nonumber\\
%
%
& = \frac{1}{2m}  \sum_{i \in [n]} \E \left[ \sign\left(\sum_{\ell \in N(i)} \Delta_iP_\ell\right)
  \cdot \sum_{\ell \in N(i)}  \Delta_iP_\ell \right]  \nonumber\\
%
& = \frac{1}{2}  \sum_{i \in [n]} \E \left|\Delta_i \inst \right|  \nonumber\\
%
& \geq \frac{1}{2} \sum_{i \in [n]}  \frac{1}{3^2}\left(  \Var[ \Delta_i \inst]
  \right)^{1/2}  \qquad (\text{using \pref{fact:khinchine-poly} on degree $2$
  polynomial  } \Delta_i \inst ) \nonumber \\
%
& \geq \frac{1}{18m} \sum_{i \in [n]} {\sqrt{\card{N(i)}}} \nonumber  \\
& \geq  \frac{1}{18} \cdot \frac{\sum_{i\in [n]} \sqrt{\card{N(i)}}}{\sum_{i\in [n]}
  \card{N(i)}} \qquad (\text{ using } m \leq \sum_{i\in [n]}
  \card{N(i)}) \\
& \geq \frac{1}{18 \sqrt{d}} \label{eq:linequalone}
\end{align}
where in the last step we used the fact that $\Var[\Delta_i \inst] = \E[\Delta_i
\inst(x)^2] - (\E[\Delta_i \inst(x)])^2 = \frac{\card{N(i)}}{m^2}$.

For terms with $|A| = 2$, we observe that their expectation is zero
since the corresponding functions are odd.
First, notice that for each $i \in [n]$, $s_i = \sign(\sum_{\ell \in N(i)}
\Delta_i P_\ell)$ is an even function of $x$, in that $s_i(x) = s_i(-x)$.
Consider a
clause $P_\ell$ over variables $S_\ell = i_1,i_2,i_3$.  Consider the term
corresponding to $A = i_1,i_2$, $B
= i_3$, namely $P_{\ell}(s_{i_1},s_{i_2},x_{i_3}) - \frac{1}{2} = b_{\ell}
s_{i_1}s_{i_2}x_{i_3}$.  Since $s_{i_1}, s_{i_2}$ are even functions
and $x_{i_3}$ is an odd function of $x$,
$P_{\ell}(s_{i_1},s_{i_2},x_{i_3})$ is an odd function, which implies
that,
$$ \E P_\ell(s_{i_1},s_{i_2},x_{i_3}) - \frac{1}{2} = 0$$
Using the same argument, we can conclude that
\begin{align}
 \E_{\ell \in [m]} \sum_{\substack{A \cup B \sse S_\ell, \\ \card{A} = 2}} \left(P_\ell(s_A,
  x_B) - \frac{1}{2} \right) = 0 \label{eq:linequaltwo}
\end{align}
%

Finally for terms with $|A| = 3$, we will use a trivial upper bound of
$1$, i.e.,
\begin{align}
 | \E_{\ell \in [m]} \sum_{\substack{A \cup B \sse S_\ell, \\ \card{A} = 3}} \left(P_\ell(s_A,
  x_B) - \frac{1}{2} \right) | \leq 1 \label{eq:linequalthree}
\end{align}
%
Using bounds \eqref{eq:nosignal}, \eqref{eq:linequalone},
\eqref{eq:linequaltwo} and \eqref{eq:linequalthree}
in the expression \eqref{eq:lin123} for $\E\inst(y)$,
\begin{align*}
 \E\inst(y) & \geq \frac{1}{2} + (1-\e)^3 \cdot 0 + \e(1-\e)^2 \cdot \frac{1}{18 \sqrt{d}}  +
  \e^2(1-\e) \cdot 0 + \e^3 \cdot (-1)\\
& \geq \frac{1}{2} + \frac{1}{216 d^{3/4}}
\end{align*}
\end{proof}
\fi


==> content/conclusion.tex <==
\section{Conclusion}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

